TRAMBA: A Hybrid Transformer and Mamba Architecture for Practical Audio and Bone Conduction Speech Super Resolution and Enhancement on Mobile and Wearable Platforms

We propose TRAMBA, a hybrid transformer and Mamba architecture for acoustic and bone conduction speech enhancement, suitable for mobile and wearable platforms. Bone conduction speech enhancement has been impractical to adopt in mobile and wearable platforms for several reasons: (i) data collection is labor-intensive, resulting in scarcity; (ii) there exists a performance gap between state of-art models with memory footprints of hundreds of MBs and methods better suited for resource-constrained systems. To adapt TRAMBA to vibration-based sensing modalities, we pre-train TRAMBA with audio speech datasets that are widely available. Then, users fine-tune with a small amount of bone conduction data. TRAMBA outperforms state-of-art GANs by up to 7.3% in PESQ and 1.8% in STOI, with an order of magnitude smaller memory footprint and an inference speed up of up to 465 times. We integrate TRAMBA into real systems and show that TRAMBA (i) improves battery life of wearables by up to 160% by requiring less data sampling and transmission; (ii) generates higher quality voice in noisy environments than over-the-air speech; (iii) requires a memory footprint of less than 20.0 MB.

==> sections/nn_evaluation_backup.tex <==
\section{Evaluation: Audio Speech Enhancement and Super Resolution}
\label{sec:superresolution_evaluation}


First, we discuss the performance of \name in context of over-the-air speech super resolution. We compare against several state-of-art audio super resolution methods, including four U-Net architectures and two GANs (Section~\ref{subsec:models_compared}).

\subsection{Training, Validation, Testing Procedure and Metrics}
\label{subsec:eval_audio_train_valid_test_procedure_metrics}

\noindent
\textbf{Dataset.} For all methods, we trained, tested, and validated on the VCTK dataset~\cite{CSTRVCTK2019}, which contains a corpus of spoken language comprising 109 native English speakers of various regional accents. Each speaker reads out approximately 400 different sentences, totaling approximately $44$ hours of data. The first 100 individuals' speech audios are utilized for training purposes, while the speech audios of the last 9 individuals are employed for the purpose of testing.

%Each speaker is recorded reading out approximately 400 different sentences, with the total duration of the speech data being approximately 44 hours.

%To train all methods, we need to generate high-low resolution audio pairs. To be more specific, Given a high resolution signal \( x = \{x_1/R_1, \dots x_{R_1 T_1}/R_1\} \) sampled at a rate \( R_1 \), we have to generate a low-resolution version \( y = \{y_1/R_2, \dots y_{R_2 T_2}/R_2\} \) of \( x \) that has a sampling rate \( R_2 < R_1 \). In this over-the-air audio super resolution task, \(R_1\) is 16kHz, \(R_2\) is 4kHz. In addition to EBEN, we utilized the default down-sampling methods specified for the other models under comparison. For EBEN, which employs a low-pass filter as its default method, we incorporated an additional down-sampling technique to it. Meanwhile, for \name, we employed the audio processing tool Sound eXchange (SoX) \cite{barras2012sox} to down-sample the audio. This adjustment ensures a consistent and comparative analysis across all models.

\noindent
\textbf{Preprocessing and Training.} For OTA speech enhancement, we downsample high resolution clean audio to $4$kHz to use as input to learn high resolution $16$kHz audio. Training data was divided into smaller segments with a window size of $512$ms and 50\% overlap. For all other methods, we applied the preprocessing steps mentioned the respective papers. We train \name for $30$ epochs. After this time period, we notice that the training, testing, and validation loss changes very little. We trained all other methods using their default training parameters specified in their respective papers and code.

\noindent
\textbf{Loss Function.} In our experiments, we found that using mean squared error (MSE) as the loss function generated lower quality audio than mean absolute error (MAE). As such, we adopted MAE as our primary loss function. However, leveraging MAE, or any type of sample-by-sample distance metric (e.g., MSE), does not necessarily guarantee perceptual quality~\cite{msenot}. As such, we also incorporate multi-resolution STFT loss \cite{yamamoto2020parallel}. We leverage the same multi-resolution STFT loss parameters as \cite{defossez2020real, mandel2023aero}: FFT bins $\in \{512, 1024, 2048\}$, hop lengths $\in \{50, 120, 240\}$, and window sizes $\in \{240, 600, 1200\}$. Our final loss is the sum between MAE and the mutli-resolution STFT loss.



%Consequently, MAE loss was selected as the baseline for the loss function. Given that MAE is not a guarantee of perceptual quality, we also utilise a multi-resolution STFT loss \cite{yamamoto2020parallel} in conjunction with the MAE loss. Similar to \cite{defossez2020real, mandel2023aero}, the multi-resolution STFT loss uses FFT bins $\in \{512, 1024, 2048\}$, hop lengths $\in \{50, 120, 240\}$, and window sizes $\in \{240, 600, 1200\}$.


\noindent
\textbf{Performance Metrics.} The primary metrics we use to compare \name for this section and throughout the rest of the paper are discussed next. %The notation used is as follows: \textcolor{red}{x.}

\noindent
\underline{Signal to Noise Ratio (SNR):} SNR serves as a metric to assess the clarity and quality of a processed audio signal relative to its background noise. SNR quantifies the level of the desired signal in comparison to the level of background noise, thereby providing an objective measure of audio fidelity. It is calculated using the formula:

\[
\text{SNR}(x, y) = 10 \log_{10} \left(\frac{\sum x^2}{\sum (x - y)^2}\right)
\]

In the formula, \( x \) represents the magnitude spectrum of the original (high resolution) signal, and \( y \) denotes the magnitude spectrum of the processed signal.


\noindent
\underline{Perceptual Evaluation of Speech Quality (PESQ):} In the context of audio super resolution, PESQ ~\cite{pesq} serves as an objective measurement to evaluate the quality of reconstructed high-resolution speech signals as perceived by human listeners. This metric compares the generated audio against a high-quality reference, with scores typically ranging from -0.5 to 4.5. A higher PESQ score indicates a closer distance to the original audio's quality.%, highlighting the effectiveness of the super resolution algorithm in enhancing perceptual speech quality.

\noindent
\underline{Log-Spectral Distance (LSD):} This metric measures the distance between the spectrum of the generated speech and the clean speech on the log scale. The difference is measured between log spectra because human hearing follows this scale\textcolor{red}{~\cite{lsd}}. Scores are calculated over all frequency bins, with lower values indicating a closer match to the reference spectrum, as shown below.

%In audio super resolution, LSD is employed to quantify the spectral accuracy of audio signals that have been enhanced from a lower to a higher resolution. By measuring the Euclidean distance between the log spectra of the super resolved audio and a high-resolution reference, LSD provides a clear metric of spectral fidelity. 

\[
\text{LSD}(x, y) = \frac{1}{T} \sum_{t=1}^T \sqrt{\frac{1}{K} \sum_{k=1}^K \left(\log X(t, k) - \log \hat{X}(t, k)\right)^2}
\]

\noindent
$X(t, k)$ denotes the magnitude spectrum of the original signal at time frame $t$ and frequency $k$. $\hat{X}(t, k)$ represents the magnitude spectrum of the super-resolved signal at the same time frame and frequency. $T$ indicates the total number of time frames, and $K$ is the total number of frequency bins.


\noindent
\underline{Short-Time Objective Intelligibility (STOI):} STOI \cite{stoi} compares the clarity and intelligibility of speech enhanced from a lower to a higher resolution against a clean reference, with scores ranging from 0 to 1. A higher STOI score, closer to 1, signifies better intelligibility, indicating that the enhanced speech is easier to understand.

%\noindent
%\underline{Word Error Rate (WER):} WER is the ratio between the number of incorrect words perceived and the total number of spoken words. To compute this metric, we input all generated speech signals into Whisper~\cite{whisper}, a state-of-the-art automatic speech recognition (ASR) model and compare with ground truth transcript.

\subsection{Models Compared}
\label{subsec:models_compared}

We compare against six additional models. Four of the models are UNet \cite{unet} structures, while the remaining two employ GAN \cite{gan} structures. 

\begin{itemize}
\item TFiLM~\cite{birnbaum2019temporal} is a UNet model that uses a recurrent neural network to alter the activations of the convolutional layers in the standard U-Net. 

\item AFiLM \cite{rakotonirina2021self} replaces the RNNs in TFiLM with self-attention. 

\item TUNet \cite{nguyen2022tunet} uses the Performer \cite{performer} achitecture as the bottleneck of the UNet model.

\item ATS-UNet \cite{li2022enabling} is a lightweight UNet model that reduces the number of parameters in the convolutional layers. 

\item EBEN \cite{hauret2023eben} is a GAN for audio speech super resolution with a lightweight generator model. 

\item Aero \cite{mandel2023aero} is a GAN that operates directly on the complex-valued frequency representation of audio. It employs two independent channels to process amplitude and phase information, circumventing the Spectral discontinuity and phase mismatch associated with high and low frequency splicing that are inherent to traditional methods. \textcolor{red}{What issues are these?}
\end{itemize}

\subsection{Performance Summary}
\label{subsec:eval_audio_performance_summary}




\begin{table}[ht]
  \centering
  
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
    \hline
     \multirow{ 2}{*}{}& \multirow{ 2}{*}{Params (M)} & Model & Inference & \multirow{ 2}{*}{SNR} & \multirow{ 2}{*}{PESQ} & \multirow{ 2}{*}{STOI} & \multirow{ 2}{*}{LSD} & \multirow{ 2}{*}{WER} \\ 
     & & Size (MB) & Time (ms) & & & & &  \\ \hline
     TFiLM~\cite{birnbaum2019temporal}& 68.2& \ 260.3& 4.6423&  13.7079&2.4349& 0.8475& 1.8667& \todo{4.06\%}\\ 
     AFiLM~\cite{rakotonirina2021self}& \ 134.7& \ 513.9& 5.5552&  11.3508&2.4658& 0.8689& 1.8665& \todo{4.61\%}\\ 
     TUNet~\cite{nguyen2022tunet}& \ 2.9& \ 11.2& 2.7550&  22.3046&2.5783& 0.9382& 0.9429& \todo{4.05\%}\\ 
     ATS-UNet~\cite{li2022enabling}& 0.1& \ 0.5& 3.4419&  12.1807& 1.5471& 0.6695& 1.5624 & \todo{12.49\%}\\ 
     EBEN~\cite{hauret2023eben}& \ 29.7& \ 113.3& 242.1341&  18.9196&2.5800& 0.8912& 1.0079& \todo{13.99\%}\\ 
     Aero~\cite{mandel2023aero}& \ 36.3& \ 138.7& 1084.5392&  22.5075&3.0136& 0.9386& 0.8102& \todo{4.14\%}\\
     \textbf{\name}& \ 5.2& \ 19.7& \textbf{2.3309}&  \textbf{23.2426}&\textbf{3.2344}& \textbf{0.9478}& \textbf{0.8271}& \todo{\textbf{6.30\%}}\\ \hline
  \end{tabular}

  \caption{Summary of performance of \name compared to existing audio super resolution methods. Inference time is measured on an NVIDIA L40 GPU processing one window of 512 ms.}
  \label{tab:superresolution_performance_summary}
\end{table}



Table~\ref{tab:superresolution_performance_summary} summarizes the test performance across all methods. We see that \name (highlighted) has the best performance across all metrics and sampling rates, while requiring similar processing times and memory as U-Net models. The Aero GAN method slightly outperforms \name in the LSD metric. LSD measures signal similarity more than perceptual quality and \name outperforms Aero in all other perceptual and noise metrics (SNR, PESQ, STOI). This demonstrates the addition of transformers and Mamba improved the modeling and generation of local speech formants than traditional U-Net architectures and encoder-decoder architectures. This also demonstrates that transformer and Mamba-based architectures can outperform state-of-art GANs with only a fraction of the memory and inference time. Both GANs require significantly more time to perform inference on an L40 GPU. Aero requires more time than the length of the window size it processes ($1080$ms vs. $512$ms), meaning it cannot run in real-time. For these reasons, we compare with the best performing U-Net architecture (TUNet) for the rest of this section.

% In the following subsections, we explore the performance of \name in more detail.






\subsection{Reducing Sampling Rate}
\label{subsec:reducing_sampling_rate}

\begin{figure}[!t]
    \centering
    \resizebox{0.8\linewidth}{!}{%
        \begin{subfigure}[b]{0.30\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/samplerate_superresolution_1.pdf}
        % \caption{subfigure caption}
        % \label{fig:figx_subfigurex}
        \end{subfigure}
        \hfill % space between subfigures
        \begin{subfigure}[b]{0.30\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/samplerate_superresolution_2.pdf}
        \end{subfigure}
        \hfill % space between subfigures
        \begin{subfigure}[b]{0.30\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/samplerate_superresolution_3.pdf}
        \end{subfigure}
    } % end resizebox
    \caption{Effects of the sampling rate on audio speech super resolution.}
    \label{fig:samplerate_superresolution}
\end{figure}

Figure~\ref{fig:samplerate_superresolution} shows the super resolution performance of \name to $16$kHz as the sampling rate of the input signal varies from 500Hz to 4kHz. Even as the sampling rate decreases down to 500Hz, \name outperforms TUNet. Even if the sampling rate decreases down to $2$kHz or $1$kHz, \name achieves comparable performance to other models at higher sampling rates.

\subsection{Super Resolution Architecture Ablation Study}
\label{subsec:architecture_ablation Study}

\begin{table}[ht]
  \centering
  \begin{tabular}{|c|c|c|c|c|c|} % 这里定义了四列，分别为左对齐、居中、右对齐和固定宽度的列
    \hline
    & PESQ& STOI& LSD& Parameter & Train Time Per Epoch \\ \hline
    Replace Mamba with Performer & 3.1208 & 0.9474 & 0.8042 & 6.5M & 243.93s \\ 
    Remove SAFiLM & 2.8056 & 0.9428 & 0.8268 & 2.6M & 114.04s \\ \hline
    TRAMBA & 3.2344 & 0.9478 & 0.8271 & 5.2M & 191.61s \\ \hline
  \end{tabular}

  \caption{Ablation study.}
  \label{tab:architecture_ablation_study}
\end{table}

Figure~\ref{tab:architecture_ablation_study} shows the results of our ablation study, which explores the impact of combining self-attention, transformers, and Mamba on speech enhancement. Replacing Mamba in our bottleneck layer with Performer, a variant of transformers, yielded similar performance metrics (PESQ, STOI, LSD). However, the training time increased significantly from 191.61 seconds to 243.93 seconds per epoch and the number of parameters increased to $6.5$M. Mamba not only maintains performance but also significantly increases model training speed and reduces the required number of model parameters.


Next, we removed attention (SAFiLM) from the contracting and expansion layers and observed that the training time per epoch decreased by more than $50$\%. However, the LSD, STOI, and particulary PESQ dropped significantly. This performance loss highlights the importance of transformers and self-attention in enabling models to learn and generate complex patterns of speech. The results of our ablation study demonstrates the importance of both self-attention and Mamba in creating a robust model for generating high quality speech, while being efficient in time and memory footprint.

%to learn intricate speech signals and enhance speech quality. The incorporation of self-attention mechanisms has been demonstrated to significantly enhance the model's capacity to process speech signals, thereby leading to the generation of more accurate and optimal results.


%In a separate ablation experiment, the impact of removing the self-attention mechanism on model performance was investigated. The results demonstrated that while the training time was reduced following the removal of self-attention, the PESQ, STOI, and LSD performance of the model declined significantly, particularly in the case of PESQ, which dropped from 3.2344 to 2.8056. This pronounced performance loss highlights the pivotal role of self-attention in enabling the model to learn intricate speech signals and enhance speech quality. The incorporation of self-attention mechanisms has been demonstrated to significantly enhance the model's capacity to process speech signals, thereby leading to the generation of more accurate and optimal results.

%The results of the ablation experiments indicate that the \name model exhibits robust performance across a range of performance indicators, effectively combining self-attention and Mamba. Additionally, the model demonstrates clear advantages in terms of time efficiency and parameter usage during model training.







%This study employs an ablation approach to evaluate the impact of combining self-attention and Mamba on audio super-resolution tasks. Several variations were designed to explore the specific impact of these two mechanisms when applied individually and jointly on model performance. The experimental results are detailed in Table \ref{tab:architecture_ablation_study}, which presents the performance of each configuration on key performance indicators such as PESQ, STOI, and LSD.

%In the experimental configuration in which Mamba was replaced by Performer, a variant of Transformer, we observed that although Performer's results were comparable to those using Mamba in terms of PESQ, STOI, and LSD indicators, the training time of the model increased from 191.61 seconds to 243.93 seconds. Additionally, the number of parameters increased from 5.2M to 6.5M. This indicates that although Performer exhibits comparable performance to Mamba, it is less time-efficient. By contrast, Mamba not only maintains performance but also significantly increases model training speed and reduces the required number of model parameters, thereby optimizing overall computing resource usage.

%In a separate ablation experiment, the impact of removing the self-attention mechanism on model performance was investigated. The results demonstrated that while the training time was reduced following the removal of self-attention, the PESQ, STOI, and LSD performance of the model declined significantly, particularly in the case of PESQ, which dropped from 3.2344 to 2.8056. This pronounced performance loss highlights the pivotal role of self-attention in enabling the model to learn intricate speech signals and enhance speech quality. The incorporation of self-attention mechanisms has been demonstrated to significantly enhance the model's capacity to process speech signals, thereby leading to the generation of more accurate and optimal results.

%The results of the ablation experiments indicate that the \name model exhibits robust performance across a range of performance indicators, effectively combining self-attention and Mamba. Additionally, the model demonstrates clear advantages in terms of time efficiency and parameter usage during model training.







\section{Evaluation: Finetuning from Audio Super Resolution to ACCEL and BCM Speech Enhancement}
\label{sec:eval_transfer_learning}

In this section, we discuss the performance of \name on enhancing speech captured by accelerometer readings and bone conduction microphones on areas of the face where (future) wearables are commonly worn. As discussed in Section~\ref{subsec:background} collecting ground truth pairs (ACCEL/BCM, audio) is extremely labor intensive. As such, we onlt fine-tune our over-the-air audio speech super resolution model (Section~\ref{sec:superresolution_evaluation}) with a small amount of paired data collected from an individual, which is similar in procedure to many existing AI voice generation applications~\cite{create2023apple}.


\subsection{Data Collection}
\label{subsec:eval_tl_data_collection}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures/data_collection.pdf}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Data collection setup, environments deployed, and wearable prototype.}
    \label{fig:datacollection_setup}
\end{figure}

We recruit 7 volunteers (4 males, 3 females) between 18-30 years old. All studies were approved by the \textit{REDACTED} IRB. We collect data from each volunteer, placing the ACCEL or BCM at each location marked in Figure~\ref{fig:datacollection_setup}a. At each location, we collect a total of approximately 20 minutes of data. We instruct each volunteer to read a set of sentences from an e-book on basic spoken English~\cite{BasicSpokenEnglish}. We vary the amount of data used to fine-tune \name to analyze the effects of the quantity of data on performance.

Figure~\ref{fig:datacollection_setup}c shows the glasses wearable we created to both collect data and deploy in various environments. There is a holder for the ACCEL/BCM to collect inputs and a holder for an over-the-air microphone to capture high resolution ground truth speech. For the BCM, we use the V2S200D voice vibration sensor~\cite{v2s2024knowles} and the IIM-42352 for the MEMS accelerometer~\cite{iim2021invensense}.


\subsection{Effects of Preprocessing: Downsampling}
\label{subsec:effects_preprocessing}


%How inputs are preprocessed can greatly affect the performance of the model. We analyze the effects of two types of preprocessing during training, as discussed in Section~\ref{subsec:background}: 1) normalizing inputs and 2) downsampling.

%\subsubsection{Normalization}
%\label{subsubsec:normalization}

\begin{comment}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures_placeholder/normalization_effects.png}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Visualization of the effects of normalization on generated outputs.}
    \label{fig:effects_normalization}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures_placeholder/normalization_effects_numbers.png}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Normalization effects on performance.}
    \label{fig:effects_normalization_numbers}
\end{figure}
\end{comment}

\begin{comment}
\begin{table*}[!t]
	\caption{Effects of normalization.}
	\centering
	\resizebox{0.5\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|}
              \cline{1-5}
              & \textbf{PESQ} & \textbf{STOI} & \textbf{LSD} & \textbf{WER} \\
		   \hline
              \hline
			 \multicolumn{5}{|c|}{Without Normalization} \\
             \hline
             \hline

             TFiLM & 0.5 & 0.6 & 1.5 & 1.5 \\
             AFiLM & 0.5 & 0.6 & 1.5 & 1.5 \\
             TUnet & 0.5 & 0.6 & 1.5 & 1.5 \\
             EBEN & 0.5 & 0.6 & 1.5 & 1.5 \\
             Aero & 0.5 & 0.6 & 1.5 & 1.5 \\
             \name & 0.5 & 0.6 & 1.5 & 1.5 \\
              \hline
              \hline
              \multicolumn{5}{|c|}{With Normalization} \\
             \hline
             \hline

             TFiLM & 0.5 & 0.6 & 1.5 & 1.5 \\
             AFiLM & 0.5 & 0.6 & 1.5 & 1.5 \\
             TUNet & 0.5 & 0.6 & 1.5 & 1.5 \\
             EBEN & 0.5 & 0.6 & 1.5 & 1.5 \\
             Aero & 0.5 & 0.6 & 1.5 & 1.5 \\
             \name & 0.5 & 0.6 & 1.5 & 1.5 \\
             \hline
		\end{tabular}
	}
	\label{tab:effects_normalization}
\end{table*}
\end{comment}

\begin{comment}
As mentioned in Section~\ref{subsec:background}, acoustic attenuation through skin and bone is significantly higher than over the air across all frequencies. As such, the energy of the vibration signals corresponding to speech will appear very low if sensed with a common inertial measurement unit that is not tuned to speech. Figure~\ref{fig:effects_normalization} shows an example phrase spoken by a person, recorded using a BCM and an ACCEL \textcolor{red}{placed at location x}. While the higher frequencies \textcolor{red}{(above x Hz)} are still attenuated in the BCM signal, the ACCEL sees even more attenuation across all frequencies. The energy of the ACCEL acceleration signal is much closer to the noise floor than to the energy level of the ground truth signal observed by the over-the-air microphone. 

As such, \textbf{for ACCELs we found significant improvements in all performance metrics if the input window is normalized} rather than using the raw signal. \textbf{For BCMs, we observed no significant performance differences with or without normalization} because the BCM already captures significant portions of speech at the lower fundamental frequencies. These observations are reflected in Figure~\ref{fig:effects_normalization_numbers}.
\end{comment}


%\subsubsection{Downsampling}
%\label{subsubsec:downsampling}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures_placeholder/downsample_effects.png}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Effects of downsampling.}
    \label{fig:effects_downsampling}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures_placeholder/downsample_effects_numbers.png}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Downsampling effects on performance.}
    \label{fig:effects_downsampling_numbers}
\end{figure}

\begin{comment}
\begin{table*}[!t]
	\caption{Effects of downsampling method.}
	\centering
	\resizebox{0.5\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|}
              \cline{1-5}
              & \textbf{PESQ} & \textbf{STOI} & \textbf{LSD} & \textbf{WER} \\
		   \hline
              \hline
			 \multicolumn{5}{|c|}{Filter + Decimate} \\
             \hline
             \hline

             TFiLM & 0.5 & 0.6 & 1.5 & 1.5 \\
             AFiLM & 0.5 & 0.6 & 1.5 & 1.5 \\
             TUnet & 0.5 & 0.6 & 1.5 & 1.5 \\
             EBEN & 0.5 & 0.6 & 1.5 & 1.5 \\
             Aero & 0.5 & 0.6 & 1.5 & 1.5 \\
             \name & 0.5 & 0.6 & 1.5 & 1.5 \\
              \hline
              \hline
              \multicolumn{5}{|c|}{Subsample} \\
             \hline
             \hline

             TFiLM & 0.5 & 0.6 & 1.5 & 1.5 \\
             AFiLM & 0.5 & 0.6 & 1.5 & 1.5 \\
             TUnet & 0.5 & 0.6 & 1.5 & 1.5 \\
             EBEN & 0.5 & 0.6 & 1.5 & 1.5 \\
             Aero & 0.5 & 0.6 & 1.5 & 1.5 \\
             \name & 0.5 & 0.6 & 1.5 & 1.5 \\
             \hline
		\end{tabular}
	}
	\label{tab:effects_downsampling}
\end{table*}
\end{comment}

As discussed in Section~\ref{subsec:background}, most works that develop super resolution methods for both over-the-air and vibration-based speech sensing 1) still sample at the non-decimated sampling rate (e.g., $16$kHz), or 2) perform low-pass filtering before subsampling. In both scenarios, aliasing is avoided or significantly reduced, but we cannot reduce power consumption by sampling at a lower rate. As such, we directly 3) decimate speech signals, without any filtering, for an accurate representation of a slower sampling rate.

Figure~\ref{fig:effects_downsampling} and Figure~\ref{fig:effects_downsampling_numbers} compares the performance of \name after downsampling from $16$kHz to \textcolor{red}{$4$kHz} with the two downsampling approaches, 2) and 3). For method 2), we apply a low-pass filter with a cut-off frequency of $2$kHz before subsampling. We see that \name outperforms other methods across all metrics. Although there is a drop in performance for \name if we remove filtering before decimation (3), \name still outperforms most other methods even if the other methods filter before decimating (2). Additionally, the performance drop-off is significantly steeper for other methods. For the rest of this section, we directly decimate audio signals, 3).



\subsection{BCM and ACCEL-based Speech Enhancement}
\label{subsec:eval_tl_bcm}

\begin{table*}[!t]
	\centering
	\resizebox{1\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
              \cline{3-10}
              \multicolumn{2}{c}{} & \multicolumn{4}{|c||}{\textbf{BCM}}& \multicolumn{4}{c|}{\textbf{ACCEL}} \\
		   \cline{3-10}
              \hline
			 Method & Fine-tuning Time Per Epoch & PESQ & STOI & LSD & \multicolumn{1}{c||}{WER} & PESQ & STOI & LSD & WER \\
             \hline

             TFiLM & 24.62s & 2.1390 & 0.8769 & 1.3342 & \multicolumn{1}{c||}{8.73\%} & 1.6577 & 0.8486 & 1.4760 & 12.89\% \\
             AFiLM & 28.45s & 2.2618 & 0.8784 & 1.4657 & \multicolumn{1}{c||}{6.48\%} & 1.6220 & 0.8422 & 1.7090 & 15.66\% \\
             TUNet & 2.65s & 1.9195 & 0.8701 & 1.1220 & \multicolumn{1}{c||}{6.21\%} & 1.6337 & 0.8366 & 1.4649 & 13.29\% \\
             ATS-UNet & 12.91s & 1.4155 & 0.7398 & 1.5370 & \multicolumn{1}{c||}{29.86\%} & 1.2981 & 0.6356 & 1.5979 & 71.80\% \\
             Aero & 29.7s & 2.6669 & 0.9072 & 0.8917 & \multicolumn{1}{c||}{4.48\%} & 2.0172 & 0.8993 & 1.1009 & 14.04\% \\
             \textbf{\name} & \textbf{1.578s} & \textbf{2.7273} & \textbf{0.9221} & \textbf{0.9329} & \multicolumn{1}{c||}{\textbf{2.65\%}} & \textbf{2.1365} & \textbf{0.9159} & \textbf{1.0326} & \textbf{7.76\%} \\
             \hline
		\end{tabular}
	}

 \caption{Performance summary of speech enhancement from $4$kHz to $16$kHz. Models were fine-tuned using \textcolor{red}{$15$ minutes of data collected at Location 2 (Nasal Bone) as shown in Figure \ref{fig:datacollection_setup} for 52 minutes.} Models were fine-tuned on an NVIDIA L40 GPU.}
 \label{tbl:eval_bcm_imu_summary}
\end{table*}

\begin{figure}[!t]
    \centering
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_a.pdf}
            \caption{Ground Truth}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_b.pdf}
            \caption{BCM Input (4kHz)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_c.pdf}
            \caption{ACCEL Input (4kHz)}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_d.pdf}
            \caption{BCM - TUNet (UNet)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_e.pdf}
            \caption{BCM - Aero (GAN)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_f.pdf}
            \caption{\textbf{BCM - \name}}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_g.pdf}
            \caption{ACCEL - TUNet (UNet)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_h.pdf}
            \caption{ACCEL - Aero (GAN)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Figures/transfer_visualization_bcm_imu_audio_i.pdf}
            \caption{\textbf{ACCEL - \name}}
        \end{subfigure}
    \caption{Visualizing reconstructed audio from ACCEL and BCM after finetuning ACCEL/BCM + audio data pairs. The BCM and ACCEL are placed at location 2 (Nasal Bone). (b) and (c) show no energy at frequencies higher than $2$kHz because the BCM and ACCEL were sampled at $4$kHz.}
    \label{fig:transfer_visualization_bcm_imu_audio}
\end{figure}


Table~\ref{tbl:eval_bcm_imu_summary} summarizes the performance of \name for speech super resolution on BCMs and ACCELs, subsampled at $4$kHz to $16$kHz sampling rate that most works benchmark. The values here represent the average performance across all participants and BCM/ACCEL placements. The models were fine-tuned on each volunteer with $15$ minutes of data at Location 2 (Nasal Bone) as shown in Figure \ref{fig:datacollection_setup} for \textcolor{red}{52 minutes}. We see that \name significantly outperforms existing methods for both sensing modalities and across all metrics. 

One additional metric we compare is the word error rate (WER), which is the ratio between the number of incorrect words perceived and the total number of spoken words. To compute this metric, we input all generated speech signals into Whisper~\cite{whisper}, a state-of-the-art automatic speech recognition (ASR) model and compare with ground truth transcript.

Compared to the larger GAN and U-Net methods, \name requires only a fraction of the time to fine-tune (\textcolor{red}{1.6 sec vs 30 sec}). Figure~\ref{fig:transfer_visualization_bcm_imu_audio} visualizes the BCM and accelerometer reconstruction result of one speech segment compared to the best performing GAN (Aero) and U-Net (TUNet). Both \name and Aero clearly generate higher quality results than TUNet. \name rectifies aliased speech better than the GAN, as evidenced at the end of the segment. The formants in the original clean speech stays level or trends upwards. However, the BCM and ACCEL are both aliased when sampled at $4$kHz. Aero reconstructs the end of the segment with the formants trending downward in the higher frequencies due to aliasing. However, \name reconstructs speech much more closely to the original speech pattern. 

Next, we explore how \name performs depending on sensor placement, across different volunteers, and availability of labeled data. For the rest of the section, we compare \name against method TUNet, as it was the second best performing method overall outside of the GANs. While the GAN architectures generally outperformed the U-Net architectures, they take orders of magnitude longer to train, fine-tune, and perform inference, making them impractical to deploy.

\subsubsection{BCM and ACCEL Placement}
\label{subsubsec:placement}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/transfer_bcm_finetuning_locations.pdf}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Performance of BCM/ACCEL speech enhancement at different locations.}
    \label{fig:transfer_bcm_finetuning_locations}
\end{figure}

Figure~\ref{fig:transfer_bcm_finetuning_locations} illustrates the performance breakdown of \name by BCM and ACCEL placement location. \name has consistent and better performance across all common and practical locations for a BCM or ACCEL.

\subsubsection{Breakdown Across Individuals}
\label{subsubsec:individuals}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/transfer_bcm_finetuning_persons.pdf}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Performance of BCM/ACCEL speech enhancement breakdown by individuals.}
    \label{fig:transfer_bcm_finetuning_persons}
\end{figure}

Figure~\ref{fig:transfer_bcm_finetuning_persons} shows the performance of \name broken down by each volunteer. The BCM and ACCEL was placed \textcolor{red}{at location 2 (Nasal Bone)}. Again, \name consistently yielded the best performance metrics across all participants. One interesting trend among all methods is that performance is lower among females than males. We suspect that this is due to their higher frequency voices experiencing greater attenuation through bone and skin. In future work, we plan to explore causes an solutions in more depth.

%with method - x, as the baseline, across all volunteers. Here, the BCM and ACCEL was placed at location - x. 

\subsubsection{Data Availability}
\label{subsubsec:data_availability}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/transfer_bcm_data_amount.pdf}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Performance of BCM/ACCEL speech enhancement varying the amount of data available to fine-tune.}
    \label{fig:transfer_bcm_data_amount}
\end{figure}

Figure~\ref{fig:transfer_bcm_data_amount} varies the amount of data we collect from an individual. \name outperforms TUNet with all fine-tuning dataset size. With only $2$ minutes of data, \name outperforms TUNet across all metrics even if TUNet was fine-tuned with $15$ minutes of data collected from the user.


%\name achieves similar performance with only \textcolor{red}{yyy min} of data compared to \textcolor{red}{TUNet with more than zzzz min of data collected from the user.}



\subsubsection{Fine-tuning Time}
\label{subsubsec:finetuning_time}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/transfer_bcm_finetuning_time.pdf}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Performance of BCM/ACCEL speech enhancement varying the number of epochs used to fine-tune.}
    \label{fig:transfer_bcm_finetune_time}
\end{figure}

Figure~\ref{fig:transfer_bcm_finetune_time} varies the number of epochs used for fine-tuning up to 2000 epochs, which corresponded to $52$ minutes of training \name. We compare \name to TUNet trained for the same amount of time. Again, \name outperforms TUNet at all training times. With only $2.6$ minutes (100 epochs) of training, \name outperforms TUNet trained for $52$ minutes across all metrics, except for PESQ, which is only slightly lower.

%We see that \name achieves better performance than \textcolor{red}{TUNet with much less training: yyy vs. zzzz minutes.}

\subsubsection{Sampling Rate}
\label{subsubsec:subsample_rate}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{Figures/transfer_bcm_samplerate.pdf}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Performance of speech enhancement, varying the the input sampling rate.}
    \label{fig:transfer_bcm_samplerate}
\end{figure}

Figure~\ref{fig:transfer_bcm_samplerate} varies the starting sampling rate to perform super resolution to $16$kHz. \name outperforms TUNet across all starting sampling rates. We observe that \name achieves acceptable speech quality when upsampling from around $2$kHz or higher for both BCM and accelerometer. TUNet only achieves similar performance as \name when the sampling rate is at least double, meaning \name can enhance and generate higher quality and resolution speech with less information, sampling, and transmission bandwidth.

%varies the sample varies the number of epochs used for fine-tuning. We see that \name achieves better performance than \textcolor{red}{xxx with much less training: yyy vs. zzzz epochs.}

\subsubsection{Unseen Individuals and the Need for Fine-Tuning}
\label{subsubsec:unseen_individuals}





%For completeness, Figure~\ref{tbl:transfer_bcm_finetuning_unseen} shows the performance of \textcolor{red}{\name on unseen individuals. Here, we fine-tune \name and TUNet .} Even though the performance of \name decreased slightly compared to fine-tuning and testing on a single user, \textcolor{red}{\name still outperforms all other methods across all metrics in this setting. This also suggests that \name could be generalizable to unseen individuals if more paired OTA and vibration-based speech from more individuals were available in the future.} 

\begin{comment}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures_placeholder/locations_finetuning_bcm.png}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Performance of BCM/ACCEL speech enhancement on unseen individuals after fine-tuning with \textcolor{red}{x volunteers} broken down at different locations.}
    \label{fig:transfer_bcm_finetuning_unseen}
\end{figure}
\end{comment}


\begin{table*}[!t]
	\centering
	\resizebox{.8\textwidth}{!}{
\begin{tabular}{|c|cccc||cccc|}
\hline
 & \multicolumn{1}{c|}{\textbf{PESQ}} & \multicolumn{1}{c|}{\textbf{STOI}} & \multicolumn{1}{c|}{\textbf{LSD}} & \textbf{WER} & \multicolumn{1}{c|}{\textbf{PESQ}} & \multicolumn{1}{c|}{\textbf{STOI}} & \multicolumn{1}{c|}{\textbf{LSD}} & \textbf{WER} \\ \hline
 & \multicolumn{4}{c||}{BCM - \name} & \multicolumn{4}{c|}{BCM - TUNet} \\ \hline
(i) Pre-train on audio only & \multicolumn{1}{c|}{1.0859} & \multicolumn{1}{c|}{0.6515} & \multicolumn{1}{c|}{1.8639} & \todo{?} & \multicolumn{1}{c|}{1.1141} & \multicolumn{1}{c|}{0.6223} & \multicolumn{1}{c|}{2.2536} & \todo{?} \\ \cline{1-1}
(ii) Creating generalizable model & \multicolumn{1}{c|}{1.1614} & \multicolumn{1}{c|}{0.7544} & \multicolumn{1}{c|}{1.1713} & \todo{?} & \multicolumn{1}{c|}{1.1130} & \multicolumn{1}{c|}{0.7239} & \multicolumn{1}{c|}{1.3392} & \todo{?} \\ \cline{1-1}
(iii) Fine-tuning to the individual & \multicolumn{1}{c|}{2.7273} & \multicolumn{1}{c|}{0.9221} & \multicolumn{1}{c|}{0.9329} & \todo{?} & \multicolumn{1}{c|}{1.9195} & \multicolumn{1}{c|}{0.8701} & \multicolumn{1}{c|}{1.1220} & \todo{?} \\ \hline
 & \multicolumn{4}{c||}{ACC - \name} & \multicolumn{4}{c|}{ACC - TUNet} \\ \hline
(i) Pre-train on audio only & \multicolumn{1}{c|}{1.1893} & \multicolumn{1}{c|}{0.7095} & \multicolumn{1}{c|}{2.1775} & \todo{?} & \multicolumn{1}{c|}{1.1590} & \multicolumn{1}{c|}{0.6714} & \multicolumn{1}{c|}{2.1154} & \todo{?} \\ \cline{1-1}
(ii) Creating generalizable model & \multicolumn{1}{c|}{1.2926} & \multicolumn{1}{c|}{0.7709} & \multicolumn{1}{c|}{1.3226} & \todo{?} & \multicolumn{1}{c|}{1.3073} & \multicolumn{1}{c|}{0.7515} & \multicolumn{1}{c|}{1.7991} & \todo{?} \\ \cline{1-1}
(iii) Fine-tuning to the individual & \multicolumn{1}{c|}{2.1365} & \multicolumn{1}{c|}{0.9195} & \multicolumn{1}{c|}{1.0326} & \todo{?} & \multicolumn{1}{c|}{1.6337} & \multicolumn{1}{c|}{0.8366} & \multicolumn{1}{c|}{1.4649} & \todo{?} \\ \hline
\end{tabular}
	}
 \caption{Performance with fine-tuning and without fine-tuning.}
	\label{tbl:with_without_finetuning}
\end{table*}

\begin{table*}[!t]
	
	\centering
	\resizebox{0.7\textwidth}{!}{
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
              \cline{2-9}
              \multicolumn{1}{c}{} & \multicolumn{4}{|c||}{\textbf{BCM}}& \multicolumn{4}{c|}{\textbf{ACCEL}} \\
		   \cline{2-9}
              \hline
			 Method & PESQ & STOI & LSD & \multicolumn{1}{c||}{WER} & PESQ & STOI & LSD & WER \\
             \hline

             TFiLM & 1.0827 & 0.6875 & 1.5167 & \multicolumn{1}{c||}{73.36\%} & 1.3512 & 0.7378 & 1.9940 & 34.31\% \\
             AFiLM & 1.0979 & 0.6903 & 1.5710 & \multicolumn{1}{c||}{72.99\%} & 1.2900 & 0.7433 & 1.9806 & 39.73\% \\
             TUNet & 1.1130 & 0.7239 & 1.3392 & \multicolumn{1}{c||}{44.52\%} & 1.3073 & 0.7515 & 1.7991 &  38.92\%\\
             ATS-UNet & 1.0967 & 0.5717 & 2.1571 & \multicolumn{1}{c||}{81.15\%} & 1.1371 & 0.6583 & 1.7805 & 76.52\% \\
             Aero & 1.1557 & 0.7084 & 1.2218 & \multicolumn{1}{c||}{54.42\%} & 1.1944 & 0.7661 & 1.4720 & 23.45\% \\
             \textbf{\name} & \textbf{1.1614} & \textbf{0.7544} & \textbf{1.1713} & \multicolumn{1}{c||}{\textbf{34.67\%}} & \textbf{1.2926} & \textbf{0.7709} & \textbf{1.3226} & \textbf{37.50\%} \\
             \hline
		\end{tabular}
	}

 \caption{Performance of BCM/ACCEL speech enhancement on unseen individuals after training with $6$ volunteers and testing on an unseen volunteer. The poor performance across all methods suggests that creating a generalizable model with a limited amount of data, due in part to the labor intensive data collection process, is not feasible. Rather, fine-tuning to specific users is currently more practical.}
 \label{tbl:transfer_bcm_finetuning_unseen}
\end{table*}





For completeness, we explore the need for fine-tuning by looking at two cases: (i) directly applying the model pre-trained on audio speech (\textcolor{red}{Section~\ref{xx}}) and (ii) creating a model for BCM and accelerometer speech that is generalizable to unseen individuals.

\noindent
\textbf{(i) Applying audio speech pre-trained model to BCM and ACCEL.} Figure~\ref{tbl:with_without_finetuning} shows the performance of the direct application of \name that is only pre-trained on downsampled audio speech (Section~\ref{xx}) to enhancing BCM and accelerometer speech. PESQ and STOI see very low values, suggesting that training \name using only OTA audio is not sufficient.

\noindent
\textbf{(ii) Creating a generalizable model.} Going one step further, we attempt to create a generalizable model by fine-tuning \name with as big of a dataset as possible. Figure~\ref{tbl:transfer_bcm_finetuning_unseen} compares \name with baseline models after training the models with most of our volunteers (6 volunteers) and testing on the unseen (1 volunteer). All methods see equally poor performance, suggesting the need for more data from more individuals to create a general model. Figure~\ref{tbl:with_without_finetuning} further highlights the disparity in performance between simply pre-training on audio (i), attempting to create a generalizable model (ii), and fine-tuning to the individual (iii). Until tools and platforms exist for collecting large amounts of paired audio and vibration data, creating and incorporating a general model is not practically feasible.







==> sections/related_works_backup.tex <==
\section{Related Works}
\label{sec:related_works}

\subsection{Audio Super-Resolution}

Audio super-resolution, also known as bandwidth expansion, refers to the restoration of high-resolution signals from low-resolution signals. Specifically, it employs the low-frequency components of the low-resolution signal to predict the high-frequency components of the signal, thereby increasing the sampling rate and improving the quality of the audio.

A lot of experiments have demonstrated that deep learning can perform audio super-resolution tasks with remarkable efficacy. Kuleshov et al. proposed TFiLM \cite{kuleshov2017audio}, the first architecture employing convolutional networks for audio super-resolution tasks. They utilized a bidirectional LSTM module to construct a variant of UNet for processing audio signal input. On this basis, Rakotonirina substituted recurrent neural networks (RNNs) with self-attention \cite{rakotonirina2021self}, thereby enhancing the perceptual quality of the output high-resolution audio. Some other deep learning methods are selected to enhance audio in the frequency domain, thus utilizing spectrograms as an input. For example, the three-layer fully connected network \cite{li2015deep} proposed by Li and Lee. In order to take advantage of both time-domain and frequency-domain signals, some researchers combine the two domains of signals. For instance, TFNet \cite{lim2018time} proposed by Lim et al. employs two networks to operate on waveforms and spectrograms simultaneously. 

Recent studies have also demonstrated the advantages of generative adversarial networks (GANs). Seanet \cite{li2021real}, EBEN \cite{hauret2023eben}, Aero \cite{mandel2023aero}, the naturalness of audio generated by these methods using GANs is relatively good. However, as GANs necessitate the integration of both generator and discriminator, these networks often exhibit a high degree of complexity, with numerous associated parameters.

It is important to acknowledge that the low-resolution signals utilized in the audio super-resolution methodologies mentioned above were generated through downsampling of the original, high-resolution signals, rather than directly collected from the low-sample-rate recording equipment.

\subsection{Multi-Modal Speech Enhancement}

Speech enhancement is a signal processing technology designed to restore clear speech from speech signals contaminated by noise, echo, or other interference. Its primary objective is to enhance the quality of speech signals, thereby improving speech clarity, intelligibility, and satisfaction. With the advent of deep learning technology, speech enhancement methods based on neural networks have made significant strides in recent years, markedly improving speech quality.

Bone conduction sensors and accelerometers are designed to record the vibrations of the wearer, thereby inherently protecting the device from ambient noise. However, their own sampling rates are often very low, which can result in the signal they record being missing high frequencies. Recent research has employed noise-free speech information from bone conduction sensors or accelerometers in conjunction with signals from air-conducting microphones to enhance speech, thereby restoring the high-frequency portion of the audio. Two different approaches have been proposed for speech enhancement. The first approach \cite{he2023towards} combines bone conduction sensors and air conduction microphones, while the second approach \cite{wang2022fusing} uses an Inertial Measurement Unit in conjunction with an air conduction microphone.

However, air conduction microphones consume a relatively high power during operation, and the aforementioned technologies all rely on their signals, so these methods generally do not have the advantage of low power consumption. Therefore, it is critical to develop technologies that rely solely on bone conduction sensors or accelerometers. In addition, most current technologies focus on a single type of sensor, and it has not been proven whether these methods can be generalized between different types of sensors. Consequently, it is also of great importance to develop technologies that can be widely applied to a variety of sensors.

\subsection{Mamba}

The challenge of enhancing long-range dependence in convolutional neural networks (CNNs) still persists. Recently, state space sequence models (SSMs) \cite{gu2021combining}, especially structured state space sequence models (S4) \cite{gu2021efficiently}, have shown outstanding performance in the analysis of continuous long sequence data. The Mamba model \cite{gu2023mamba}nhas advanced S4 by incorporating a selection mechanism that enables the model to choose relevant information based on the input. This enhancement makes Mamba particularly adept at handling pattern-intensive tasks like language processing. Motivated by these strengths of SSMs and Mamba, we are exploring the possibility of employing the Mamba module to develop models tailored for audio super-resolution tasks.





==> sections/superresolution_backup.tex <==
\section{Audio Super Resolution Architecture Design}
\label{sec:superresolution}



In this section, we introduce the rationale behind the design of audio super resolution DNN. \textcolor{red}{Detail the flow of the rest of the section, namely what each subsection will describe.}

\subsection{Opportunities and Challenges}
\label{subsec:background}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures_placeholder/audio_imu_bcm_downsampling.png}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Comparison of audio, imu, and BCM recorded audio under different sampling and filtering schemes.}
    \label{fig:imu_bcm_audio_visualization}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures_placeholder/performance_efficiency.png}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Comparison of performance vs efficiency of \name and state-of-art audio super resolution methods. Each metric described in Section~\ref{subsec:eval_audio_train_valid_test_procedure_metrics} is scaled between 0 (worst performing) to 1 (best performing) and averaged to obtain the `performance' metric shown in these graphs. \textcolor{red}{The alternative to doing this averaging is to replicate these graphs for each metric or a select number of them.}}
    \label{fig:performance_vs_efficiency}
\end{figure}

Audio and speech super resolution refers to the task of predicting and generating higher frequency components for lower resolution audio to improve sound quality. For speech, this involves predicting higher frequency `formants’, or high concentrations of energy around specific frequency bands, given lower formants sensed at lower frequencies. \textcolor{red}{Figure~\ref{fig:imu_bcm_audio_visualization}xxx-xxx} show an example of speech (time series and spectrogram) collected from an OTA microphone, a BCM, and the acceleration experienced by an IMU \textcolor{red}{placed at xxxxxx}. We see that the higher frequencies and formants on the vibration-based sensors (BCM and IMU) are severely attenuated compared to the OTA microphone. 

Figure~\ref{fig:performance_vs_efficiency} compares the performance and efficiency between \name and six different state-of-art audio super resolution methods, which can broadly be categorized into two approaches: 1) U-Net models and 2) GAN models. U-Net models consist of contracting layers that compress the input into a lower dimensional latent space before expanding back out again. This allows the network to learn important low dimensional features in the lower frequencies before generating higher frequency content in the expansive layers. GANs consist of a generator network that attempts to learn and generate audio waveforms that are indistinguishable from real data by discriminator network. From Figure~\ref{fig:performance_vs_efficiency}, we see several trends and challenges preventing practical adoption of speech super resolution for bone conduction sensors.



\subsubsection{Heavy Performance and Performance Gap}
\label{subsubsec:heavy_performance}

The general trend is that the best performing models (GANs) orders of magnitude more memory (tens of billions vs. billions of parameters and hundreds of MBs vs MBs), training time (days or weeks vs. minutes), and fine-tuning time than U-Net architectures. However, pure U-Net architectures that are more amenable to resource constrained mobile and wearable platforms see significantly worse performance.

\subsubsection{Data Scarcity}
\label{subsubsec:data_scarcity}

Training \name or any bone conduction-based super resolution method requires inputs collected from the BCM or accelerometer/IMU, paired with speech collected from OTA microphones that can capture higher frequency formants and act as ground truth. This paired data is not readily available, unlike pure speech or audio collected that can be collected with only a single microphone. Most works that specifically focus on speech enhancement for bone conduction or vibration-based microphones collect a sizeable amount of data from several volunteers to train/test models, and the datasets are generally not publicly available~\cite{x}. Other works artificially simulate bone conduction microphones and learn transformations to convert large datasets of audio collected by OTA microphones into signals that you might observe on an IMU or BCM~\cite{x}, which is used to train the model. However, such methods need to be carefully tuned to generate data that appropriately captures the characteristics of signal observed by an IMU or BCM at different sensor locations and different people. Methods trained in this way have difficulty generalizing to new users and sensor placements.

On the other hand, works that focus on OTA audio super resolution need to train and test only on standard speech and audio datasets~\cite{x}. These works can easily generate realistic inputs by manually attenuating higher frequency components by applying low pass filters, allowing them to take advantage of the vast amount of publicly available audio. We find that directly applying models trained in this way on OTA speech signals produces poor super resolution results (Section~\ref{sec:eval_transfer_learning}). As shown in \textcolor{red}{Figure~\ref{fig:imu_bcm_audio_visualization}xxx-xxx}, low pass filtering OTA audio does not produce signals comparable to those sensed through vibration due to differences in signal pathway between these modalities (skin and bone vs. air).

\subsubsection{System Design Opportunities}
\label{subsubsec:system_design_opportunities}

The general trend in energy-efficient systems research is to perform computation as close to the edge as possible (e.g., on the wearable or earable recording audio). This is because the output in many detection, classification, and recognition tasks is much lower in dimension than the input. This significantly reduces the amount of data needed to transmit wirelessly and improves battery life. In this work, we aim to produce high resolution audio (16 kHz). This means if the model runs on the wearable platform, we still need to transmit full high resolution audio to the mobile platform, meaning power consumption from wireless transmission cannot be reduced. Moreover, general purpose microcontrollers (MCU) and system-on-chips (SoC) that typically comprise earable and wearable platforms currently cannot support models larger than tens or hundreds of KB~\cite{x}, which limits the performance of models that can be incorporated.

From \textcolor{red}{Figure~\ref{fig:imu_bcm_audio_visualization}xxx-xxx}, we see that most of the higher frequencies above \textcolor{red}{x Hz} for both the BCM and IMU have extremely low energy. This suggests that we can aggressively reduce the sampling rate from the IMU and BCM to reduce power consumption of sampling. Moreover, if model inference and fine-tuning occurs on the mobile platform, the wearable can also reduce the activity of its wireless radio and significantly improve battery life. Moreover, a mobile platform like a smartphone typically has more compute and battery life than a wearable, allowing us to leverage bigger and better performing models.

However, most works that focus on audio super resolution still sample at high sampling rates, such as in \textcolor{red}{Figure~\ref{fig:imu_bcm_audio_visualization}xxxxx} (e.g., 16 kHz), and attempt to fill in higher frequencies~\cite{x}. Works that operate on lower sampling frequency inputs tend to low pass filter before decimating the signal, which avoids aliasing, as shown in \textcolor{red}{Figure~\ref{fig:imu_bcm_audio_visualization}xxxxx}. However, this still requires sampling at a high data rate, which does not improve power consumption on the sensing front. To achieve savings on both sampling and transmission fronts, we aim for robust acoustic super resolution on signals that are directly subsampled at a lower frequency rather than filtered signals that have been decimated from higher sampling rates.

\subsection{Deep Neural Network Architecture}
\label{subsec:dnn_architecture}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.90\linewidth]{Figures/network_architecture.png}
    %\includesvg[inkscapelatex=false,width=0.90\linewidth]{Figures_new/system_architecture.svg}
    %\vspace{-10px}
    \caption{Super resolution architecture.}
    \label{fig:dnn_network_architecture}
\end{figure}

Our neural network architecture is designed based on \cite{kuleshov2017audio,perez2018film,rakotonirina2021self}. The overall structure is shown in Figure \ref{fig:dnn_network_architecture}.

\subsubsection{Down-Sampling Block}

Our model comprises a total of three downsampling blocks, each of which performs convolution, LeakyReLU, and Scale-only Attention-based Feature-wise Linear Modulation(SAFiLM). Downsampling block \textit{b} = 1, 2, 3 contains $2^{5+\textit{b}}$ convolutional filters and a stride of 4. The convolution kernel sizes of each convolution layer are 65, 17, and 7 respectively.

\subsubsection{SAFiLM}

The neural network layer of Scale-only Attention-based Feature-wise Linear Modulation(SAFiLM) is employed based on FiLM \cite{perez2018film} and AFiLM \cite{rakotonirina2021self}. Like AFiLM \cite{rakotonirina2021self}, SAFiLM replaced the RNN in FiLM \cite{perez2018film} with a self-attention mechanism functioning as a FiLM generator, thereby exclusively scale the activations of the convolutional model and capturing long-range dependencies.

Analogous to AFiLM \cite{rakotonirina2021self}, The modulation of SAFiLM is conducted on the level of feature map blocks too. In this method, T and C are the one-dimensional space dimension and the number of channels respectively. The initial activations \( F \), shaped as \( \mathbb{R}^{T \times C} \), are segmented into \( B \) individual blocks. Each block is represented as \( F_{\text{block}} \), and subsequently undergoes dimensionality reduction along its temporal axis via max pooling to form \( F_{\text{pool}} \).

Unlike AFiLM\cite{rakotonirina2021self}, in order to further reduce the parameters of the overall model, this adaptation is executed without the use of translation parameters, relying solely on a scaling mechanism. Within this framework, each block's scaling parameters, \( \gamma \), are synthesized by the Transformer Block, which is composed of stacked multi-head self-attention and dense layers, augmented by residual paths and normalization strategies. The equation governing the block-wise scaling is expressed as:
\begin{equation}
    \gamma[b, :] = \text{TransformerBlock}(F_{\text{pool}}[b, :])
\end{equation}
wherein the activations undergo modulation through scaling, mathematically formulated as:
\begin{equation}
    \text{SAFiLM}(F_{\text{block}}[b, t, c]) = \gamma[b, c] \times F_{\text{block}}[b, t, c]
\end{equation}
This approach omits the translational element, focusing on modulating activation magnitudes and preserving the inherent distribution of the feature maps. The SAFiLM mechanism, predicated solely on scaling effects, aims to impact feature maps across any length, maintaining cognizance of overarching interconnections.

\subsubsection{Bottleneck}

In our model structure, we utilize Mamba \cite{gu2023mamba} as our bottleneck. We posit that this approach will confer certain advantages. For instance, the Mamba model exhibits exemplary performance when processing long sequence data, particularly its capacity to retain pertinent information and discard irrelevant data. We hypothesize that this capability can facilitate the efficient handling of data with long-distance dependencies by UNet models. Additionally, the Mamba model is designed with hardware efficiency in mind, especially in terms of performance on GPUs. This implies that when Mamba is employed as a bottleneck, UNet models may achieve accelerated computation speeds during training and inference, particularly when confronted with large-scale data sets.

\subsubsection{Up-Sampling Block}

As with the downsampling blocks, our model also comprises three upsampling blocks, each of which performs convolution, dropout, LeakyReLU, pixelshuffle, and SAFiLM. With regard to the upsampling block preceding the final output, it should be noted that it performs only convolution and pixelshuffle. 

For pixelshuffle layer, we also implement a one-dimensional version of \cite{shi2016real} like \cite{kuleshov2017audio}. If the input of the pixelshuffle layer is ($C_{\text{in}}$, $T_{\text{in}}$) and the scaling factor is 4, the output is ($C_{\text{in}}$ $\div$ 4, $T_{\text{in}}$ $\times$ 4). Upsampling block \textit{b} = 1, 2, 3 contains 512, 256, 4 convolutional filters respectively, and a stride of 4. The convolution kernel sizes of each convolution layer are 7, 17, and 65 respectively.

\subsubsection{Residual Connection}

Instead of using Skip Connection, we add residual connection directly to \textit{b}-th downsampling features and the (3 - \textit{b} + 1)-th tensor of upsampling features. Furthermore, a residual connection is established between the input and the final output.



\subsection{Fine-tuning}
\label{subsec:transfer_learning}

As mentioned in Section~\ref{subsec:background}, it is labor intensive to obtain large amounts of paired bone conduction data and clean audio to train a robust model for vibration-based speech enhancement. Rather than take this approach, we instead pre-train our model using \textcolor{red}{the xxx speech dataset} before fine-tuning with a small amount of paired data collected from the user at box opening. To pre-train the model, we downsample clean speech to use as input. During fine-tuning, the clean speech can be captured the user's mobile phone, while the wearable records from the BCM or IMU simultaneously.
